Planets in Globular Clusters?

The discovery of planets around PSR~1257+12 suggests that planetary systems may be detected around the recycled pulsars found in globular clusters. Planetary systems in dense clusters have lifetimes to disruption due to perturbations by passing stars comparable to or shorter than the pulsar lifetime, and observations of planets in the cores of clusters may reveal planetary systems formally dynamically unstable on time scales short compared to the characteristic age, $\tau_c$, of the system. Planets formed around cluster pulsars will most likely be restricted to semi--major axis of $\sim 0.1-1.0\, AU$, while "scavenged" planets may be observed in wider orbits, with no stable systems expected in the densest clusters. Observation is most probable in the cluster rich high--density pre-core collapse clusters such as 47Tuc. Detection of planets around cluster pulsars can constrain planet formation mechanisms, in particular the effects of low metallicity on planet formation in disks.

==> qmsfont.tex <==
%  Define \...point macros to change fonts and spacings consistently
\catcode`@=11
\chardef\@ne=1
\chardef\tw@=2
\newdimen\z@ \z@=0pt% can be used both for 0pt and 0
%
\def\tenpoint{
\def\rm{\fam\z@\tenrm}
\textfont0=\tenrm \scriptfont0=\sevenrm \scriptscriptfont0=\fiverm
\textfont1=\teni \scriptfont1=\seveni \scriptscriptfont1=\fivei
\textfont2=\tensy \scriptfont2=\sevensy \scriptscriptfont2=\fivesy
\textfont3=\tenex \scriptfont3=\tenex \scriptscriptfont3=\tenex
\textfont\itfam=\tenit \def\it{\fam\itfam\tenit}% \it is family 4
\textfont\slfam=\tensl \def\sl{\fam\slfam\tensl}% \sl is family 5
\textfont\ttfam=\tentt \def\tt{\fam\ttfam\tentt}% \tt is family 7
\textfont\bffam=\tenbf \scriptfont\bffam=\sevenbf
\scriptscriptfont\bffam=\fivebf \def\bf{\fam\bffam\tenbf}% \bf is family 6
\def\mit{\fam\@ne}\def\oldstyle{\fam\@ne\teni}
\def\cal{\fam\tw@}
\setbox\strutbox=\hbox{\vrule height8.5pt depth3.5pt width0pt}
\normalbaselineskip=12pt
\parskip=0pt plus 1pt
  \abovedisplayskip 12pt plus 3pt minus 9pt
  \belowdisplayskip 12pt plus 3pt minus 9pt
  \abovedisplayshortskip 0pt plus 3pt
  \belowdisplayshortskip 7pt plus 3pt minus 4pt
  \smallskipamount=3pt plus1pt minus1pt
  \medskipamount=6pt plus2pt minus2pt
  \bigskipamount=12pt plus4pt minus4pt
\normalbaselines\rm}
%
%  Define a whole menagerie of pseudo-12pt fonts
     
\font\twelverm=cmr10 scaled 1200    \font\twelvei=cmmi10 scaled 1200
\font\twelvesy=cmsy10 scaled 1200   \font\twelveex=cmex10 scaled 1200
\font\twelvebf=cmbx10 scaled 1200   \font\twelvesl=cmsl10 scaled 1200
\font\twelvett=cmtt10 scaled 1200   \font\twelveit=cmti10 scaled 1200
\skewchar\twelvei='177   \skewchar\twelvesy='60
     
\def\twelvepoint{
\def\rm{\fam\z@\twelverm}
\textfont0=\twelverm \scriptfont0=\tenrm \scriptscriptfont0=\sevenrm
\textfont1=\twelvei \scriptfont1=\teni \scriptscriptfont1=\seveni
\textfont2=\twelvesy \scriptfont2=\tensy \scriptscriptfont2=\sevensy
\textfont3=\twelveex \scriptfont3=\twelveex \scriptscriptfont3=\twelveex
\textfont\itfam=\twelveit \def\it{\fam\itfam\twelveit}% \it is family 4
\textfont\slfam=\twelvesl \def\sl{\fam\slfam\twelvesl}% \sl is family 5
\textfont\ttfam=\twelvett \def\tt{\fam\ttfam\twelvett}% \tt is family 7
\textfont\bffam=\twelvebf \scriptfont\bffam=\tenbf
\scriptscriptfont\bffam=\sevenbf \def\bf{\fam\bffam\twelvebf}% \bf is family 6
\def\mit{\fam\@ne}\def\oldstyle{\fam\@ne\teni}
\def\cal{\fam\tw@}
\setbox\strutbox=\hbox{\vrule height10.2pt depth4.2pt width0pt}
\normalbaselineskip=14.4pt
\parskip=0pt plus 1pt
  \abovedisplayskip 14.4pt plus 3.6pt minus 10.8pt
  \belowdisplayskip 14.4pt plus 3.6pt minus 10.8pt
  \abovedisplayshortskip 0pt plus 3.6pt
  \belowdisplayshortskip 8.4pt plus 3.6pt minus 4.8pt
  \smallskipamount=3.6pt plus1.2pt minus1.2pt
  \medskipamount=7.2pt plus2.4pt minus2.4pt
  \bigskipamount=14.4pt plus4.8pt minus4.8pt
\normalbaselines\rm}
%
\catcode`@=12% at signs are no longer letters
     
%fonts for headings etc.
     
\font\titlefnt=cmbx10 scaled 1728
\font\sc=cmcsc10 scaled 1200
\font\secfnt=cmbx10 scaled 1440
\font\subfnt=cmsl10 scaled 1440



